Riesz-Quincunx-UNet Variational Auto-Encoder for Satellite Image Denoising

Multiresolution deep learning approaches, such as the U-Net architecture, have achieved high performance in classifying and segmenting images. However, these approaches do not provide a latent image representation and cannot be used to decompose, denoise, and reconstruct image data. The U-Net and other convolutional neural network (CNNs) architectures commonly use pooling to enlarge the receptive field, which usually results in irreversible information loss. This study proposes to include a Riesz-Quincunx (RQ) wavelet transform, which combines 1) higher-order Riesz wavelet transform and 2) orthogonal Quincunx wavelets (which have both been used to reduce blur in medical images) inside the U-net architecture, to reduce noise in satellite images and their time-series. In the transformed feature space, we propose a variational approach to understand how random perturbations of the features affect the image to further reduce noise. Combining both approaches, we introduce a hybrid RQUNet-VAE scheme for image and time series decomposition used to reduce noise in satellite imagery. We present qualitative and quantitative experimental results that demonstrate that our proposed RQUNet-VAE was more effective at reducing noise in satellite imagery compared to other state-of-the-art methods. We also apply our scheme to several applications for multi-band satellite images, including: image denoising, image and time-series decomposition by diffusion and image segmentation.

==> bios.tex <==
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_pictures/Duy_headshot.png}}] {Duy H. Thai} is a researcher at George Mason University, USA, at the Department of Geography and Geoinformation Science.
He received his Ph.D. in Institute for Mathematical Stochastics, University of Goettingen, Germany, with Prof. A. Munk. Then, he was a researcher at Duke University, USA, at the Department of Statistical Science.
Dr. Thai's research focuses on harmonic analysis, optimization and stochastic calculus applied in image processing, machine learning and stochastic dynamical systems.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_pictures/Tri_photo.jpg}}] {Minh Tri Le} is a Ph.D student at George Mason University, USA, at the Department of Geography and Geoinformation Science. His research focuses on the applications of machine learning and deep learning approaches on remote sensing data, and methods for geospatial data management and visualization.
\end{IEEEbiography}



\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_pictures/Andreas_headshot_bowtie.jpg}}] {Andreas Z\"ufle} is an acting associate professor at Emory University, USA, at the Department of Computer Science. He received his Ph.D. in Computer Science at Ludwig Maximilian University of Munich, Germany (LMU), in 2013. Dr. Z\"ufle's research focuses on data management. He is mainly known for his contribution to the field of geospatial data management and mining. In this area, he has made contributions in several subareas, notably uncertain data management, spatial indexing, clustering, and geosimulation. His interdisciplinary work has applications in geosciences, transportation, epidemiology, and social science.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{author_pictures/Konrad Wessels crop.png}}] {Konrad Wessels} is an Associate Professor in the Department of Geography and Geoinformation Science of George Mason University, USA. He received his PhD in the Geographical Sciences from University of Maryland on a NASA Earth System Sciences Fellowship. He previously served as Chief Scientist and Group Leader of the Remote Sensing Research Unit within the Council for Scientific and Industrial Research (CSIR), CSIR-Meraka Institute for Information and Communication Technology, South Africa. He is a remote sensing expert with applications in land cover change, savanna ecology, human settlement monitoring, fire, carbon cycle modelling and biomass estimation. He is a member of the NASA Carbon Monitoring System Science Team.  
\end{IEEEbiography}








==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> subsections/background.tex <==

%\section{Background}%Appendix?  
%\label{sec:Background}
%

%
\subsection{Notations and Definitions:}
\label{sec:NotationsDefinitions}
%
%
The following list provides an overview of notations used throughout this work.
\begin{itemize}
 %
 \item continuous coordinate in the spatial domain: $x = (x_1 \,, x_2) \in \mathbb R^2$,
 
 %
 \item discrete coordinate in the spatial domain: $k = (k_1 \,, k_2) \,, m = (m_1 \,, m_2) \in \mathbb Z^2$,
 
 %
 \item Fourier coordinate: $\omega = (\omega_1 \,, \omega_2) \in [-\pi \,, \pi]^2$,
 
 %
 \item Complex number: $j = \sqrt{-1}$, 

 %
 \item Image domain: $\Omega = \{ 1 \,, \ldots \,, n_1 \} \times \{ 1 \,, \ldots \,, n_2 \}$, $\abs{\Omega} = n_1 \times n_2$,
 
 %
 \item Images and stacks of images:
  
  %
  \begin{itemize}
   %
   \item a gray-scale image $\underline{f} = \begin{pmatrix} f_1 & \hdots &  f_{n_2} \end{pmatrix} \in \mathbb R^{\abs{\Omega}} \,, f_i \in \mathbb R^{n_1}$, 
   
   %
   \item a multi-channel image $\underline{\underline{f}} = \left\{ \underline{f_1} \,, \hdots \,, \underline{f_{P}} \right\} \in \mathbb R^{\abs{\Omega} \times P} \,, \underline{f_i} \in \mathbb R^{\abs{\Omega}}$,
    
   %
   \item a set of observed images $\textfrak{F} := \underline{\underline{\underline{f}}} = \left\{ \underline{\underline{f_i}} \right\}_{i=1}^T \in \mathbb R^{\abs{\Omega} \times P \times T}$,
  \end{itemize}

 %
 \item Distribution and Lebesgue density: $\underline{f} \stackrel{\text{i.i.d.}}{\sim} \mathbb{P}\left( \underline{f} \right) := \mathbb{P}\left( \text{d} \underline{f} \right) = \mathtt{p}\left( \underline{f} \right) \text{d}\underline{f}$,
 
 
 \item Continuous Fourier transform of a continuous function $a \in L_2(\mathbb R^2)$ is:
\begin{align*}
 a(x) &\stackrel{\cF}{\longleftrightarrow} 
 \widehat{a}(\omega) = \int_{\mathbb R^2} a(x) e^{-j \langle x \,, \omega \rangle_{\ell_2} } \text{d} x \,,
\end{align*} 
%
and its discrete version is computed via Poisson summation formulae:
\begin{align*}
 a[k] &:= a(x) \mid_{x = k \in \mathbb Z^2} 
 \\  % ----
 \stackrel{\cF}{\longleftrightarrow} 
 \widehat{A} \left( e^{j \omega} \right) &= \sum_{k \in \mathbb Z^2} a[k] e^{-j \langle k \,, \omega \rangle_{\ell_2} } 
 %
 = \sum_{k \in \mathbb Z^2} \widehat{a}(2 \pi k + \omega) \,.
\end{align*}
%
Additional definitions can be found in the supplemental material.


%
%Given a sampling matrix $\text{D}$, a space decomposition is
%\begin{align}  \label{eq:SpaceDecomposition}
% \mathbb Z^2 = \bigcup_{l=0}^{\abs{\text{det(D)}} - 1} \left\{ \text{D}^\text{T} \mathbb Z^2 + \widehat{\rho}_l \right\} \,,~ \widehat{\rho}_l \in \left\{ \text{D}^\text{T} t \,:\, t \in [0 \,, 1)^2 \right\} \,.
%\end{align}

\end{itemize}



% -----


==> subsections/images.tex <==
% \section*{Appendix A. Images}
%

% ======================================

%
\clearpage

% =============================================
%

% =============================================





%
%\begin{figure}
%\begin{center}  

% Original:
%\subfigure[Training error]{\includegraphics[width=0.5\textwidth]{UnetVAE_TrainingError.png}}

%
%\caption{This plot illustrates a training error of the loss function of the proposed RQUnet-VAE with 500 images fot training. Since high order Riesz-Quincunx wavelet is an identity operator, the training procedure is only applied for Unet-VAE. This figure shows that the algorithm has a good convergence.  
%}
%\label{fig:TrainingErrorLoss:2019059hdf}
%\end{center}
%\end{figure}

% ===========================================


% =============================================
%

% =============================================


% ============================================
\begin{figure*}
\begin{center}  

%
\subfigure[Original image]{\includegraphics[width=0.24\textwidth]{figures/ImageDenoising_originalimage1.png}}
%
\subfigure[Noisy image, $\text{std} = 0.04$]{\includegraphics[width=0.24\textwidth]{figures/ImageDenoising_noisyimage1.png}}
%
\subfigure[Denoised image]{\includegraphics[width=0.24\textwidth]{figures/ImageDenoising_denoisedimage1.png}}
%
\subfigure[Relative error]{\includegraphics[width=0.24\textwidth]{figures/ImageDenoising_RelativeError1.png}}

% Skip-connecting signals of noisy image at scale 0
\subfigure[scale 0, subband 0]{\includegraphics[width=0.19\textwidth]{figures/ImageDenoising_SkipConnectingNoisyImage1_scale0direction0.png}}
%
\subfigure[subband 1]{\includegraphics[width=0.19\textwidth]{figures/ImageDenoising_SkipConnectingNoisyImage1_scale0direction1.png}}
%
\subfigure[subband 2]{\includegraphics[width=0.19\textwidth]{figures/ImageDenoising_SkipConnectingNoisyImage1_scale0direction2.png}}
%
\subfigure[subband 3]{\includegraphics[width=0.19\textwidth]{figures/ImageDenoising_SkipConnectingNoisyImage1_scale0direction3.png}}
%
\subfigure[subband 4]{\includegraphics[width=0.19\textwidth]{figures/ImageDenoising_SkipConnectingNoisyImage1_scale0direction6.png}}
%
%\subfigure[subband 5]{\includegraphics[width=0.19\textwidth]{ImageDenoising_SkipConnectingNoisyImage1_scale0direction7.png}}

% %
% \subfigure[subband 4]{\includegraphics[width=0.24\textwidth]{ImageDenoising_SkipConnectingNoisyImage1_scale0direction4.png}}
% %
% \subfigure[subband 5]{\includegraphics[width=0.24\textwidth]{ImageDenoising_SkipConnectingNoisyImage1_scale0direction5.png}}


% Skip-connecting signals of smoothed image at scale 0
%
%\vspace{-0.4cm}
\subfigure[scale 0, subband 0]{\includegraphics[width=0.19\textwidth]{figures/ImageDenoising_SkipConnectingSmoothedImage1_scale0direction0.png}}
%
\subfigure[subband 1]{\includegraphics[width=0.19\textwidth]{figures/ImageDenoising_SkipConnectingSmoothedImage1_scale0direction1.png}}
%
\subfigure[subband 2]{\includegraphics[width=0.19\textwidth]{figures/ImageDenoising_SkipConnectingSmoothedImage1_scale0direction2.png}}
%
\subfigure[subband 3]{\includegraphics[width=0.19\textwidth]{figures/ImageDenoising_SkipConnectingSmoothedImage1_scale0direction3.png}}
% %
% \subfigure[subband 4]{\includegraphics[width=0.19\textwidth]{ImageDenoising_SkipConnectingSmoothedImage1_scale0direction4.png}}
% %
% \subfigure[subband 5]{\includegraphics[width=0.19\textwidth]{ImageDenoising_SkipConnectingSmoothedImage1_scale0direction5.png}}
%
\subfigure[subband 4]{\includegraphics[width=0.19\textwidth]{figures/ImageDenoising_SkipConnectingSmoothedImage1_scale0direction6.png}}
%
%\subfigure[subband 5]{\includegraphics[width=0.19\textwidth]{ImageDenoising_SkipConnectingSmoothedImage1_scale0direction7.png}}


%
\caption{Image denoising and some skip-connecting signal of noisy images and denoised images at scale 0. A relative error shows a convergence of the algorithm. These skip-connecting images are generated by Unet-VAE; then, high order Riesz-Quincunx wavelet is applied to smoothed these signals. The model parameter $\beta$ is trained from ground-truth images. 
}
\label{fig:ImageDenoising:SkipConnectingSignal}
\end{center}
\end{figure*}
% =============================================



% ============================================

% =============================================


% ============================================

% ===========================================


% ===========================================

% ===========================================


% ============================================

% =============================================


% Image Diffusion ======================================

%

% =======================================================


%
\begin{figure*}
\begin{center}  

% Frame 1:
% Original
\subfigure[Original frame 1]{\includegraphics[width=0.22\textwidth]{figures/site6616_frame1_1.png}}
% Lowpass
\subfigure[Lowpass]{\includegraphics[width=0.22\textwidth]{figures/site6616_frame1_4.png}}
% Bandpass
\subfigure[Bandpass]{\includegraphics[width=0.22\textwidth]{figures/site6616_frame1_5.png}}
% Highpass
\subfigure[Highpass]{\includegraphics[width=0.22\textwidth]{figures/site6616_frame1_6.png}}


\vspace{-0.3cm}
% Frame 30:
% Original
\subfigure[Original frame 30]{\includegraphics[width=0.22\textwidth]{figures/site6616_frame30_1.png}}
% Lowpass
\subfigure[Lowpass]{\includegraphics[width=0.22\textwidth]{figures/site6616_frame30_4.png}}
% Bandpass
\subfigure[Bandpass]{\includegraphics[width=0.22\textwidth]{figures/site6616_frame30_5.png}}
% Highpass
\subfigure[Highpass]{\includegraphics[width=0.22\textwidth]{figures/site6616_frame30_6.png}}

% % Frame 60:
% % Original
% \subfigure[Original frame 30]{\includegraphics[width=0.24\textwidth]{site6616_frame60_1.png}}
% % Lowpass
% \subfigure[Lowpass]{\includegraphics[width=0.24\textwidth]{site6616_frame60_4.png}}
% % Bandpass
% \subfigure[Bandpass]{\includegraphics[width=0.24\textwidth]{site6616_frame60_5.png}}
% % Highpass
% \subfigure[Highpass]{\includegraphics[width=0.24\textwidth]{site6616_frame60_6.png}}

% Frame 90:
% Original

\vspace{-0.3cm}
\subfigure[Original frame 90]{\includegraphics[width=0.22\textwidth]{figures/site6616_frame90_1.png}}
% Lowpass
\subfigure[Lowpass]{\includegraphics[width=0.22\textwidth]{figures/site6616_frame90_4.png}}
% Bandpass
\subfigure[Bandpass]{\includegraphics[width=0.22\textwidth]{figures/site6616_frame90_5.png}}
% Highpass
\subfigure[Highpass]{\includegraphics[width=0.22\textwidth]{figures/site6616_frame90_6.png}}


\vspace{-0.3cm}
% Lowpass + Bandpass
% Frame 1:
\subfigure[Lowpass + Bandpass for frame 1]{\includegraphics[width=0.22\textwidth]{figures/site6616_frame1_2.png}}
% Frame 30:
\subfigure[Lowpass + Bandpass for frame 30]{\includegraphics[width=0.22\textwidth]{figures/site6616_frame30_2.png}}
% Frame 90:
\subfigure[Lowpass + Bandpass for frame 90]{\includegraphics[width=0.22\textwidth]{figures/site6616_frame90_2.png}}


% \subfigure[Histogram]{\includegraphics[width=0.32\textwidth]{site6616_frame1_3.png}}

% \includegraphics[width=1\textwidth]{Fig15.png}

\vspace{-0.3cm}
\caption{Video Decomposition by RQUnet-VAE with GIAF based spectral decomposition for site 6616. Parameters: threshold for histogram in spectral decomposition is 5, number with iterations is 10.}
\label{fig:Video Decomposition:site6616}
\end{center}
\end{figure*}


% -----
%


% ===========================================


%
\clearpage
\newpage

%
\section*{Appendix B. Tables and Algorithms}
%


% ===========================================
\newpage
\clearpage

%

% ======================

% \begin{table}[h!]
% \begin{center}
% \begin{tabular}{cccccc}
%  \toprule
%  &
%  \\
%  \multirow{2}{c}{RQUnet-VAE scheme 3}
%  %
%  \\
%  \multirow{2}{c}{RQUnet-VAE scheme 1} 
%  %
% %  \\ \cmidrule(r){3-4}\cmidrule(l){5-6}
% %  Image Set  &\#Images  &PSNR &SSIM  &PSNR &SSIM
% \end{tabular}
% %
% \caption{PSNR and SSIM: Mean $\pm$  standard deviation over the three image sets (best in bold).}
% \label{MeanVariance Comparison}
% \end{center}
% \end{table}





% \begin{tabular}{ccccc}
%  \toprule
%  &\multicolumn{2}{c}{Set A}
%  &
%  \multicolumn{2}{c}{Set B} \\\cmidrule(r){2-3}\cmidrule(l){4-5}
%  Dates &Weight& Diameter    & Weight &Diameter      \\
%  \bottomrule
% \end{tabular}




% --------------------------------------





==> subsections/init.tex <==
%\ProvidesPackage{init}
\usetikzlibrary{quotes,arrows.meta}
\usetikzlibrary{positioning}

\def\edgecolor{rgb:blue,4;red,1;green,4;black,3}
\newcommand{\midarrow}{\tikz \draw[-Stealth,line width =0.8mm,draw=\edgecolor] (-0.3,0) -- ++(0.3,0);}

\usepackage{Ball}
\usepackage{Box}
\usepackage{RightBandedBox}


